Language Preservation Problems in Parametric Timed Automata

Parametric timed automata (PTA) are a powerful formalism to model and reason about concurrent systems with some unknown timing delays. In this paper, we address the (untimed) language- and trace-preservation problems: given a reference parameter valuation, does there exist another parameter valuation with the same untimed language, or with the same set of traces? We show that these problems are undecidable both for general PTA and for the restricted class of L/U-PTA, even for integer-valued parameters, or over bounded time. On the other hand, we exhibit decidable subclasses: 1-clock PTA, and 1-parameter deterministic L-PTA and U-PTA. We also consider robust versions of these problems, where we additionally require that the language be preserved for all valuations between the reference valuation and the new valuation.

==> TPS-nondet.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Language and Trace Preservation Synthesis for Nondeterministic 1-Clock PTA}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ea{une fois encore, mon algo marche en général, c'est juste qu'il ne termine pas forcément :) À mettre avant ?}


We define below homogeneous parametric connected components, as connected sets of symbolic states of uniform parametric constraint in the zone graph of a PTA.

%------------------------------------------------------------
\begin{definition}[\HPCC{}]
	Given a PTA~$\A$, a \emph{homogeneous parametric connected component} (\HPCC{}) is a maximal connected subgraph of the zone graph of~$\A$ such that the projection onto the parameters of all constraints associated to the states of this subgraph is the same.
\end{definition}
%------------------------------------------------------------

For example, consider the zone graph of an example PTA given in \cref{figure:HPCC:example}.
This zone graph contains 5 \HPCC{}s, that is the parametric constraint is the same in each of these \HPCC{}s.
Since an \HPCC{} is a maximal subgraph, \HPCC{}s 1, 2, 3 all have parametric constraints necessarily different with each other.
Furthermore, from \cref{lemma:k-stricter}, the parametric constraints of \HPCC{}s 3 and 5 are also necessarily different with each other.
However, it could happen that the parametric constraints of \HPCC{}s 4 and 5 are the same.

\ea{TODO: define \HPCC{} graph}
An \emph{abstract path} of~$\A$ is a path in the \HPCC{} graph of~$\A$, \ie{} an alternating sequence of \HPCC{}s and edges.
An abstract path of~$\A$ is said to be \emph{valid} if it corresponds to a concrete path, \ie{} for each $(\edge_i, \hpcc_i, \edge_{i+1})$ there is a path in $\hpcc_i$ from $\edge_i$ to $\edge_{i+1}$.

For example, in \cref{figure:HPCC:example} the abstract path $\hpcc_1, \edge_3, \hpcc_3, \edge_5, \hpcc_4$ is not valid because there is no path in $\hpcc_3$ from $\edge_3$ to $\edge_5$.

\ea{TODO: prove that the graph of the \HPCC{} is a directed acyclic graph?}



%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%
\begin{figure}[t]
	\centering
	\begin{tikzpicture}[scale=1.5, ->, >=stealth', auto, thin]
	
		\tikzstyle{HPCCname}=[draw=none,font=\bf]
		\tikzstyle{HPCCtrans}=[thick]

		\node[location, initial] (s1) at (0,0) {$\loc_0$};
		\node[location] (s2) at (1,0) {$\loc_1$};
		\node[location] (s3) at (2,0) {$\loc_0$};
		\node[location] (s4) at (3,0) {$\loc_2$};
		\node[location] (s5) at (3,-1) {$\loc_1$};
		\node[location] (s6) at (1,-2) {$\loc_2$};
		\node[location] (s6') at (1,-1) {$\loc_4$};
		\node[location] (s7) at (3,-2) {$\loc_2$};
		\node[location] (s8) at (4,0) {$\loc_3$};
		\node[location] (s9) at (5,0) {$\loc_5$};
		\node[location] (s10) at (4,-1) {$\loc_4$};

		\path
			(s1) edge[] node {$a$} (s2)
			(s1) edge[HPCCtrans,bend right] node {\begin{tabular}{c}$b$\\$\edge_1$\end{tabular}} (s6)
			(s2) edge[loop above] node (selfs2) {$b$} (s2)
			(s2) edge[HPCCtrans] node {\begin{tabular}{c}$a$\\$\edge_2$\end{tabular}} (s3)
			(s2) edge[HPCCtrans] node {\begin{tabular}{c}$a$\\$\edge_3$\end{tabular}} (s6')
			(s3) edge[bend left] node (s3s4) {$b$} (s4)
			(s3) edge[bend right] node {$a$} (s5)
			(s4) edge[bend left] node {$c$} (s3)
			(s4) edge[HPCCtrans] node {\begin{tabular}{c}$c$\\$\edge_7$\end{tabular}} (s8)
			(s5) edge[] node {$b$} (s4)
			(s5) edge[HPCCtrans] node {\begin{tabular}{c}$a$\\$\edge_6$\end{tabular}} (s7)
			(s6) edge[] node[] {$a$} (s6')
			(s6) edge[HPCCtrans] node[below] {\begin{tabular}{c}$b$\\$\edge_5$\end{tabular}} (s7)
			(s6') edge[HPCCtrans,below] node {\begin{tabular}{c}$b$\\$\edge_4$\end{tabular}} (s5)
			(s7) edge[loop right] node (s7self) {$a$} (s7)
			(s8) edge[] node {$c$} (s9)
			(s8) edge[] node {$b$} (s10)
% 			(s9) edge[] node {$c$} (s10)
			(s10) edge[loop right] node {$a$} (s10)
			;
		
		% DRAW ALL HPCCs
		\begin{pgfonlayer}{background}
			\filldraw [draw,line width=4mm,join=round,orange!15]
			(s1.west |- selfs2) rectangle (s2.east |- s2.south);
		\end{pgfonlayer}
		\node[HPCCname] at (s1 |- selfs2) {1};

		\begin{pgfonlayer}{background}
			\filldraw [draw,line width=4mm,join=round,blue!15]
			(s3.west |- s3s4) rectangle (s5.east |- s5.south);
		\end{pgfonlayer}
		\node[HPCCname] at (s3 |- s5.north) {2};
  	
		\begin{pgfonlayer}{background}
			\filldraw [draw,line width=4mm,join=round,red!15]
			(s6.west |- s6.north) rectangle (s6'.east |- s6'.south);
		\end{pgfonlayer}
		\node[HPCCname,xshift=-10] at (s6.west) {3};
  	
		\begin{pgfonlayer}{background}
			\filldraw [draw,line width=4mm,join=round,green!15]
			(s7.west |- s7.north) rectangle (s7self |- s7.south);
		\end{pgfonlayer}
		\node[HPCCname,xshift=10] at (s7self.east) {4};
  	
		\begin{pgfonlayer}{background}
			\filldraw [draw,line width=4mm,join=round,green!15]
			(s8.west |- s8.north) rectangle (s9.east |- s10.south);
		\end{pgfonlayer}
		\node[HPCCname] at (s9 |- s10) {5};
  	
	\end{tikzpicture}
	\caption{Set of \HPCC{}s in an example zone graph}
	\label{figure:HPCC:example}
\end{figure}
%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%-%

%------------------------------------------------------------
\begin{definition}[set of valid abstract paths leading to an \HPCC{}]
	Given an \HPCC{} $\hpcc$, we denote by $\VAPaths(\hpcc)$ the set of valid abstract paths from the initial \HPCC{} to $\hpcc$.
\end{definition}
%------------------------------------------------------------

Note that, if the zone graph is finite, then $\VAPaths(\hpcc)$ is finite, since the \HPCC{} graph is acyclic.

For example, in \cref{figure:HPCC:example}, $\VAPaths(\hpcc_4)$ contains the following abstract paths:
\begin{enumerate}
	\item $\hpcc_1, \edge_1, \hpcc_3, \edge_4, \hpcc_2, \edge_6, \hpcc_4$
	\item $\hpcc_1, \edge_1, \hpcc_3, \edge_5, \hpcc_4$
	\item $\hpcc_1, \edge_2, \hpcc_2, \edge_6, \hpcc_4$
	\item $\hpcc_1, \edge_3, \hpcc_3, \edge_4, \hpcc_2, \edge_6, \hpcc_4$
\end{enumerate}



%------------------------------------------------------------
\begin{definition}[final language of an \HPCC{}]
	Given an \HPCC{} $\hpcc$ and an edge~$\edge_i$ going in $\hpcc$, the final language of $\hpcc$ entering via $\edge_i$, denoted by $\FinalLang(\hpcc, \edge_i)$, is the maximal language of the subgraph defined by $\hpcc$ starting from~$\edge_i$.
\end{definition}
%------------------------------------------------------------

For example, in \cref{figure:HPCC:example}, we have (we assume that $\edge_0$ is the initial edge to $\Lang(\hpcc_1)$ -- considered as an edge for sake of simplicity):
% 	let $\edge_0$ be the initial edge to $\Lang(\hpcc_1)$ (considered as an edge for sake of simplicity),
% 	let $\edge_1$ be the edge from $\Lang(\hpcc_1)$ to $\Lang(\hpcc_2)$,
% 	let $\edge_2$ be the edge from $\Lang(\hpcc_1)$ to $\Lang(\hpcc_3)$,
% 	let $\edge_3$ be the edge from $\Lang(\hpcc_2)$ to $\Lang(\hpcc_4)$,
% 	let $\edge_4$ be the edge from $\Lang(\hpcc_3)$ to $\Lang(\hpcc_2)$.
% 	and let $\edge_5$ be the edge from $\Lang(\hpcc_2)$ to $\Lang(\hpcc_5)$.
% Then:
\begin{enumerate}
	\item $\FinalLang(\hpcc_1, \edge_0) = a b^\omega$
	\item $\FinalLang(\hpcc_2, \edge_2) = (abc|bc)^\omega$
	\item $\FinalLang(\hpcc_2, \edge_4) = bc(abc|bc)^\omega$
	\item $\FinalLang(\hpcc_3, \edge_1) = a$
	\item $\FinalLang(\hpcc_3, \edge_3) = \epsilon$
	\item $\FinalLang(\hpcc_4, \edge_5) = \FinalLang(\hpcc_4, \edge_6) = a^\omega$
	\item $\FinalLang(\hpcc_5, \edge_7) = c|ba^\omega$
\end{enumerate}




%------------------------------------------------------------
\begin{definition}[traversing language of an \HPCC{}]
	Given an \HPCC{} $\hpcc$, an edge~$\edge_i$ going in $\hpcc$ and an edge~$\edge_o$ going out from $\hpcc$, we define the traversing language of $\hpcc$ for $\edge_i$ and $\edge_o$, denoted by $\TravLang(\hpcc, \edge_i, \edge_o)$, as the set of finite words that can be read from the entry into $\hpcc$ via $\edge_i$ until the exit via $\edge_o$.
\end{definition}
%------------------------------------------------------------

In \cref{figure:HPCC:example}, we have:
\begin{enumerate}
	\item $\TravLang(\hpcc_1, \edge_0, \edge_1) = \epsilon$
	\item $\TravLang(\hpcc_1, \edge_0, \edge_2) = \TravLang(\hpcc_1, \edge_0, \edge_3) = a b^*$
	\item $\TravLang(\hpcc_2, \edge_2, \edge_7) = b (c(b|ab))^*$
	\item $\TravLang(\hpcc_2, \edge_1, \edge_6) = (bc)^*a (b(cb)^*a)^*$
\end{enumerate}


%------------------------------------------------------------
\begin{definition}[language of a valid abstract path]
	Let $\hpcc$ be an \HPCC{} and $\vap$ be a valid abstract path in $\VAPaths(\hpcc)$ of the form
		$\hpcc_1, \edge_1, \ldots, \edge_{n-1}, \hpcc_{n-1}, \edge_n, \hpcc_n$.
	The language of $\vap$, denoted by $\Lang(\vap)$, is:
	
	$\TravLang(\hpcc_1, \edge_0, \edge_1) \lgconc \action_1 \lgconc \ldots \lgconc \action_{n-1} \lgconc \TravLang(\hpcc_{n-1}, \edge_{n-1}, \edge_{n}) \lgconc \FinalLang( \hpcc_n, \edge_n)$,
	where $\action_i$ is the action associated with $\edge_i$.
\end{definition}
%------------------------------------------------------------

\ea{ah ben non, il fallait rajouter les blocages intermédiaires, et prendre toutes les combinaisons…}

\ea{warning! attention aux invariants bloquants ! (ou est-ce qu'on les vire de la déf du langage ??)}

%------------------------------------------------------------
\begin{definition}[full language of an \HPCC{}]
	\ea{todo: full language reaching an \HPCC{} and ending there (including earlier blockings??)}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{definition}[synthpath(path to \HPCC{})]
	\ea{todo}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{definition}[synth(\HPCC{})]
	\ea{todo: constraint synthesized characterizing an \HPCC{} (including earlier blockings??)}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{proposition}[synth(\HPCC{}) is correct]
	\ea{todo}
\end{proposition}
%------------------------------------------------------------


%------------------------------------------------------------
\begin{definition}[combination of \HPCC{}s]
	\ea{todo}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{definition}[language associated with a combination of \HPCC{}s]
	\ea{todo}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{definition}[synth(\HPCC{})]
	\ea{todo: constraint synthesized characterizing a combination of \HPCC{}s}
\end{definition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{proposition}[synth(comb \HPCC{}) is correct]
	\ea{todo}
\end{proposition}
%------------------------------------------------------------

%------------------------------------------------------------
\begin{proposition}[synth(\HPCC{})]
	\ea{correctness and completeness of the combinations of \HPCC{}s}
\end{proposition}
%------------------------------------------------------------

\ea{hence the following algorithm:
	\begin{enumerate}
		\item synthesize all \HPCC{}s together with their associated constraint
		\item consider all combinations of \HPCC{}s
		\item compute their language and associated constraint
		\item take the union of all constraints associated with combinations of \HPCC{} the language of which is the same as $\valuate{\A}{\pval}$
	\end{enumerate}
}



\ea{\\
************************************************************\\
ce qui suit est vieux}


In the remainder of this section, we briefly address the problem of language preservation synthesis for deterministic PTA, and then the language and preservation synthesis for non-necessarily deterministic PTA.


% 
% %------------------------------------------------------------
% \begin{theorem}[language preservation synthesis]\label{theorem:language-preservation-synthesis}
% 	Let $\A$ be a deterministic 1-clock PTA and $\pval$ be a parameter valuation.
% 	It is possible to compute \ea{computable?} the set of parameters for which the language is the same as in $\valuate{\A}{\pval}$.
% \end{theorem}
% %------------------------------------------------------------
% \begin{proof}
% 	Since $\A$ is deterministic, the trace set can be obtained from the language, and in fact there is a bijection between the set of traces and the set of (untimed) words.
% 	Hence the result directly follows from \cref{theorem:trace-preservation-synthesis}.
% \end{proof}
% %------------------------------------------------------------

% \ea{ce qui suit est encore un peu brouillon, à discuter}


The non-deterministic case can be solved by taking the union of the different path constraints that correspond to the same traces (once more, since the parametric graph is finite, there is only a finite number of such combinations).


%------------------------------------------------------------
\begin{theorem}[trace preservation synthesis]\label{theorem:trace-preservation-synthesis:nondet}
	Let $\A$ be a 1-clock PTA and $\pval$ be a parameter valuation.
	It is possible to compute \ea{computable?}
	\begin{enumerate}
		\item the set of parameters for which the trace set is the same as in $\valuate{\A}{\pval}$, and 
		\item the set of parameters for which the language is the same as in $\valuate{\A}{\pval}$.
	\end{enumerate}
\end{theorem}
%------------------------------------------------------------
\begin{proof}
	\begin{enumerate}
		\item For the trace preservation in nondeterministic PTA, we need to redefine $\synthTrace(\A, \trace)$ so that it returns the union of the constraints associated with all possible occurrences of~$\trace$ in the parametric zone graph; although there may be several such traces, the number of constraints is finite, because the number of strictly connected components is finite, because the parametric zone graph is finite (\cref{theorem:finiteness-zone-graph}).
		Then, the rest of the algorithm remains unchanged.
		\item For the language preservation in nondeterministic PTA, we reuse the same reasoning as above but, this time, we need to consider at \cref{algo:TPSynth1:good:begin} in \cref{algo:TPSynth1} the union of all traces corresponding to an untimed word of $\valuate{\A}{\pval}$.
		\ea{mais là, petit problème car l'ensemble des traces est potentiellement infini… il vaut mieux adapter $\synthTrace(\A, \trace)$ aux mots…}
		\ea{JE SUIS LA}
	\end{enumerate}
\end{proof}
%------------------------------------------------------------


%------------------------------------------------------------
\begin{corollary}[trace and language preservation emptiness]
	Let $\A$ be a 1-clock PTA and $\pval$ be a parameter valuation.
	It is possible to decide whether there exists a parameter valuation $\pval' \neq \pval$ such that $\valuate{\A}{\pval}$ and $\valuate{\A}{\pval'}$ have the same trace sets (resp.\ the same language).
\end{corollary}
%------------------------------------------------------------
\begin{proof}
	From \cref{theorem:trace-preservation-synthesis:nondet}.\ea{et rajouter qqc sur le test du vide d'un polyèdre ?}
\end{proof}
%------------------------------------------------------------



% The non-deterministic case can be solved \ea{how?? Again by taking the union of the different path constraints that correspond to the same language? Is that finite??}


\begin{remark}
	In fact, the result in this section extend to complex parametric expressions in guards and invariants, i.e., to sets of parametric linear terms over $\Param{}$ (with integer coefficients) compared to either the (unique) clock or 0; in this latter case, we obtain fully parametric inequalities, rarely allowed in the syntax of PTA in the literature.
	In that case, the form of \ea{blablablabla}
\end{remark}
 

